Aesthetic Preference Prediction in Interior Design: Fuzzy Approach

Interior design is all about creating spaces that look and feel good. However, the subjective nature of aesthetic preferences presents a significant challenge in defining and quantifying what makes an interior design visually appealing. The current paper addresses this gap by introducing a novel methodology for quantifying and predicting aesthetic preferences in interior design. Our study combines fuzzy logic with image processing techniques. We collected a dataset of interior design images from social media platforms, focusing on essential visual attributes such as color harmony, lightness, and complexity. We integrate these features using weighted average to compute a general aesthetic score. Our approach considers individual color preferences in calculating the overall aesthetic preference. We initially gather user ratings for primary colors like red, brown, and others to understand their preferences. Then, we use the pixel count of the top five dominant colors in the image to get the color scheme preference. The color scheme preference and the aesthetic score are then passed as inputs to the fuzzy inference system to calculate an overall preference score. This score represents a comprehensive measure of the user's preference for a particular interior design, considering their color choices and general aesthetic appeal. We used the 2AFC (Two-Alternative Forced Choice) method to validate our methodology, achieving a notable hit rate of 0.7. This study can help designers and professionals better understand and meet people's interior design preferences, especially in a world that relies heavily on digital media.

==> ToDo.tex <==
1. Correcting Introduction - 60%
2. Describe Related Work
3. Methods
3a. Find the Instagram page
3b. Download 100 photos add to Excel file with likes for every photo
3c. Find the Lightness of 100 photos with some Python code - algorithm found, need to find brightness for 100 img
3d. add results to Excel
3e. Find the symmetry of every photo and add to excel
3f. Find complexity and add to file 
3g. Describe getting each input in an article
4. Fuzzify with rules 4 inputs(Color harmony, complexity, lightness, symmetry) find aesthetic assessment of every photo - describe it
5. ML algorithm  find correlation
6. conclusion
7. Find journal 
8. add the journal latex
9. correct to the journal latex template
10. fuzzy partition
11. input /outputs
Journal Options



aesthetic rating 
2AFC
Which visual features are essential for determining aesthetic appeal?
• To what extent can this approach give aesthetic assessment for interior design?


15 января дедлайн 
0. Гугл коллаб, убрать fig 5 done
1. КАкие свойства еще есть hue count, saturation, contrast, symmetry,
2. Посчитать корреляцию для них
3. Фаззи правила вместе 
4. Эксперименты:
2AFC, Ranking 
сравнить с 


==> name.tex <==
ADD
\textcolor{BrickRed}{} 

CORRECT
\colorbox{Dandelion}{orange background}

IDEA
\colorbox{Lavender}{IDEa is great}

{\color{RubineRed} hello

\rule{\linewidth}{0.5mm}}


By analyzing random forest regressor algorithm I conducted my own algorithm. Step by step description:
\begin{enumerate}

\item First, I run through the dataset from the interior pictures, pick 1 photo
\item Run through pixels and determine main 3 color from the picture
%\begin{figure}[htbp]
%\centerline{\includegraphics{Fig/color.jpg}}
%\caption{Example: color scheme of interior design, picked main 3 colors }
%\label{fig}
%\end{figure}
\item After run through this 3 colors in 3 list which was based on survey analysis: 
\begin{enumerate}
            \item List "Color" contains ID of color and it's popularity score. For example: white - 5, brown - 2.
            \item List "Color gradation" finds is this color suits with this 2 colors.
            \item List "Lightning" contains boolean notation like if the picture of interior design is bright then 1 , if no then 0.
\end{enumerate}            
   
\item Then, go through every color in the Color list and give score for each color. List have 3 category and scoring: 
\begin{enumerate}
\item Most popular color - 5
\item Neutral color - 3
\item Unused color - 1
\end{enumerate}

\item Compare the color with the Color gradation palette, it gives yes or no result 1 or 0 score, also provides list of suitable colors for this image.
\item Ligthing list gives 1 or 0 ball looking at the brightness of the photo, after that we sum all scores for each interior design image.
\item After that running 1000 images in dataset this algorithm can find average score of aesthetic photo and determine aesthetic score.
For instance, let's consider an array of scores representing the aesthetic assessment of interior designs: [14, 30, 34, 56, 70]. The average value of this array is calculated to be 40.8, which serves as the threshold for determining aesthetic appeal. We can compare each individual score to this average value to assess the aesthetic quality of the corresponding interior design.

For example, the picture with ID 1 received a score of 14, which is lower than the average of 40.8. Based on this comparison, we can conclude that this particular interior design is considered less aesthetic. On the other hand, the interior design image with ID 5 obtained a score of 70, which is higher than the average. Consequently, we can infer that this interior design is aesthetically pleasing and more preferred.

By utilizing the average score as a reference point, we can effectively evaluate the aesthetic appeal of different interior designs. Scores below the average indicate lower aesthetic quality, while scores above the average signify higher aesthetic appeal and desirability.
 \end{enumerate}


